Rydberg Atomic Quantum Satellites for Enhanced Ground-to-Space Direct Uplink Access

This paper investigates the performance advantages of Rydberg atomic quantum (RAQ)-based multiple-input multiple-output (MIMO) satellites for enhancing direct ground-to-space uplink access.We analytically evaluate the impact of Rydberg atoms on channel estimation by deriving closed-form expressions for the mean-square error (MSE) and normalized mean-square error (NMSE). Based on the estimated channels, we further derive lower bounds on the achievable data rates for maximum ratio combining (MRC) and zero-forcing (ZF) detection schemes. Rigorous analysis demonstrates that RAQ-MIMO outperforms conventional radio-frequency (RF) MIMO under both Rayleigh and satellite channel conditions. Specifically, compared with conventional MIMO, RAQR achieves a ``squaring" gain under Rayleigh fading, especially in long-distance transmission scenarios with stringent power constraints. In contrast, under line-of-sight (LoS)-dominated satellite channels, this gain saturates as channel-estimation benefits diminish, with the remaining improvement primarily arising from the normalized noise background. Monte Carlo simulations validate the analytical results and show that the performance gains of RAQ-MIMO satellites translate into smaller antenna apertures, lower transmit power, and longer communication ranges, thereby paving the way for next-generation satellite networks.

==> proof.tex <==
\begin{appendices}
\section{Proof of Theorem \ref{MRC_SINR_T}}
\label{Prooftheorem1}

From (\ref{kth_SINR}), we need to derive the expressions of ${\left| {{\rm{DS}}_{k}} \right|^2}$, $\mathbb{E}\left( \left| {{\rm{LS}}_{k}} \right|^2 \right)$, $\mathbb{E}\left( \left| {{\rm{UI}}_{k,k'}} \right|^2 \right)$ and $\mathbb{E}\left( \left| {{\rm{N}}_{k}} \right|^2 \right)$, respectively.

We first rewrite the expression of the estimated channel \(\mathbf{\hat h}_{m,k}\) as
\begin{equation}
    \label{rwestimatedchennel}
    \begin{split}
    \mathbf{\hat h}_{m,k} &= \sqrt{\frac{{\bar K}_{m,k}}{{\bar K}_{m,k}+1}}\sqrt{\beta_{m,k}}\mathbf{\bar{h} }_{m,k} + \sqrt{\tau p_k^p}\mathbf{R}_{m,k}\boldsymbol{\Psi}_{m,k} \Big(\sum_{j \in \mathcal{P}_k}\sqrt{\frac{\tau p^p_j\beta_{m,j}  }{{\bar K}_{m,j}+1}}\mathbf{\widetilde h}_{m,j} +{\bf{n}}_{m,k}^p \Big) \\
    & = {{\sqrt{\bar K_{m,k}a_{m,k}}\mathbf{\bar{h} }_{m,k}}}  + \underbrace{\sqrt{\tau p_k^p}\mathbf{R}_{m,k}\boldsymbol{\Psi}_{m,k}\Big(\sum_{j \in \mathcal{P}_k}\sqrt{\tau p^p_j a_{m,j}}\boldsymbol{\Delta}_{m,j}^{\frac{1}{2}}\mathbf{\widetilde h}_{m,j} +{\bf{n}}_{m,k}^p \Big)}_{\mathbf{\widetilde q}_{m,k}}.
    \end{split}
\end{equation}
The channel \(\mathbf{ h}_{m,k}\) can be rewritten as
\begin{equation}
    \mathbf{ h}_{m,k} = \sqrt{\bar K_{m,k}a_{m,k}}\mathbf{\bar{h} }_{m,k} + \sqrt{a_{m,k}}\boldsymbol{\Delta}_{m,k}^{\frac{1}{2}} \mathbf{\widetilde h}_{m,k}.
\end{equation}

Then, we compute ${\rm{DS}}_k$. Since estimated channel $\hat {\bf{h}}_{m,k}$ and estimation error $\mathbf{h}_{m,k}-\hat {\bf{h}}_{m,k}$ are independent, we have
\begin{equation}
\label{MRC_DSk}
\begin{split}
	{{\rm{DS}}_{k}}  &= { \mathbb{E}{\left\{ {\sum\limits_{m \in {\mathcal{M}}_k} { {{w_{m,k}p_k^d}} {{ {{\bf{\hat h}}^H_{m,k}} }} {{\bf{\hat h}}_{m,k}}} } \right\}} }  \\
	 &= {\sqrt{p_k^d}}  \sum\limits_{m \in {\mathcal{M}}_k} {w_{m,k}}\left\{ \tau p^p_k \text{tr}\{\mathbf{R}_{m,k}\boldsymbol{\Psi}_{m,k}\mathbf{R}_{m,k}\} + {\bar K}_{m,k}a_{m,k}||\mathbf{\bar{h} }_{m,k}||^2\right\} \\
\end{split}
\end{equation}

 Here, we note that \(\mathbf{\hat h}_{m,k}\) and \(\mathbf{\hat h}_{m,k'}\) are correlated if \(\{k,k'\} \in \mathcal{P}_k\). Therefore, we separately derive the interference's expression. First, if the \(k'\)-th user does not share the same pilot with the user \(k\), i.e., \(\{k,k'\} \notin \mathcal{P}_k\), then \(\mathbf{\hat h}_{m,k}\) and \(\mathbf{h}_{m,k'}\) are independent and we have
 \begin{equation}
\label{MRC_UIkk1}
\begin{split}
 &\mathbb{E} \left( {{{\left| {{\rm{U}}{{\rm{I}}_{k,k'}}} \right|}^2}} \right)\\
 =  &\mathbb{E} \left\{ {{{\left| {\sum\limits_{m \in {\mathcal{M}}_k} {w_{m,k}\sqrt {p_{k'}^d} {{\left( {{{{\bf{\hat h}}}_{m,k}}} \right)}^H}{{\bf{h}}_{m,k'}}} } \right|}^2}} \right\} \\
  =& {p_{k'}^d}\Big( \sum\limits_{m \in \mathcal{M}_k} w_{m,k}\sqrt{\bar K_{m,k}a_{m,k}\bar K_{m,k'}a_{m,k'}}\mathbf{\bar h}^H_{m,k}\mathbf{\bar{h} }_{m,k'} + w_{m,k}\sqrt{{\bar K}_{m,k'}a_{m,k'}}\mathbf{\widetilde q}^H_{m,k} \mathbf{\bar h}_{m,k'}\\
  + &w_{m,k}\sqrt{{\bar K}_{m,k}a_{m,k} a_{m,k'}} \mathbf{\bar h}^H_{m,k} \boldsymbol{\Delta}^{\frac{1}{2}}_{m,k'} \mathbf{\widetilde h}_{m,k'} +w_{m,k}\sqrt{a_{m,k'}}\mathbf{\widetilde q}^H_{m,k} \boldsymbol{\Delta}^{\frac{1}{2}}_{m,k'} \mathbf{\widetilde h}_{m,k'}\Big)^2\\
   =&  p^d_{k'} \left|\sum\limits_{m \in {\mathcal{M}}_k} w_{m,k}\sqrt{\bar K_{m,k}\bar K_{m,k'}a_{m,k}a_{m,k'}}\mathbf{\bar h}^H_{m,k}\mathbf{\bar h}^H_{m,k'}\right|^2 \\
   +& p^d_{k'} \mathbb{E}\left\{ \left| \sum\limits_{m \in \mathcal{M}_k} w_{m,k}\sqrt{\bar K_{m,k'}a_{m,k'}}\mathbf{\widetilde q}^H_{m,k}\mathbf{\bar h}_{m,k'}\right|^2\right\} \\
  + &  p^d_{k'} \mathbb{E}\left\{ \left|\sum\limits_{m \in {\mathcal{M}}_k}  w_{m,k}\sqrt{{\bar K}_{m,k}a_{m,k} a_{m,k'}} \mathbf{\bar h}^H_{m,k}\boldsymbol{\Delta}_{m,k'} \mathbf{\widetilde h}_{m,k'} \right|^2\right\}\\ + & p^d_{k'} \mathbb{E}\left\{ \left| \sum\limits_{m \in {\mathcal{M}}_k} w_{m,k}\sqrt{a_{m,k'}}\mathbf{\widetilde q}^H_{m,k} \boldsymbol{\Delta}_{m,k'}^{\frac{1}{2}}\mathbf{\widetilde h}_{m,k'} \right|^2\right\}
 \end{split}
 \end{equation}

\begin{equation}
    \begin{split}
        \mathbb{E}\left\{ \left| \sum\limits_{m \in \mathcal{M}_k} w_{m,k}\sqrt{\bar K_{m,k'}a_{m,k'}}\mathbf{\widetilde q}_{m,k}\mathbf{\bar h}_{m,k'}\right|^2\right\} &= \sum\limits_{m \in \mathcal{M}_k}w^2_{m,k} \bar K_{m,k'}a_{m,k'}\mathbb{E}\{\mathbf{\widetilde q}^H_{m,k}\mathbf{\bar h}_{m,k'}\mathbf{\bar h}^H_{m,k'} \mathbf{\widetilde q}_{m,k}\} \\
        & = \sum\limits_{m \in \mathcal{M}_k} w^2_{m,k}\bar K_{m,k'}\tau p^p_k a_{m,k'} \mathbf{\bar h}^H_{m,k'} \mathbf{R}_{m,k}\boldsymbol{\Psi}_{m,k} \mathbf{R}_{m,k}\mathbf{h}_{m,k'}.
    \end{split}
\end{equation}

\begin{equation}
    \begin{split}
        &\mathbb{E}\left\{ \left|\sum\limits_{m \in {\mathcal{M}}_k}  w_{m,k}\sqrt{{\bar K}_{m,k}a_{m,k} a_{m,k'}} \mathbf{\bar h}^H_{m,k} \boldsymbol{\Delta}^{\frac{1}{2}}_{m,k'} \mathbf{\widetilde h}_{m,k'} \right|^2\right\}\\
        = &\sum\limits_{m \in \mathcal{M}_k} w^2_{m,k}\bar K_{m,k}a_{m,k}a_{m,k'}\mathbb{E}\{\mathbf{\bar h}^H_{m,k}\boldsymbol{\Delta}^{\frac{1}{2}}_{m,k'} \mathbf{\widetilde h}_{m,k'}\mathbf{\widetilde h}^H_{m,k'}\boldsymbol{\Delta}^{\frac{1}{2}}_{m,k'}  \mathbf{\bar h}_{m,k}\} \\
        = &\sum\limits_{m \in \mathcal{M}_k} w^2_{m,k}\bar K_{m,k}a_{m,k}a_{m,k'}\mathbf{\bar h}^H_{m,k}\boldsymbol{\Delta}_{m,k'} \mathbf{\bar h}_{m,k}.
    \end{split}
\end{equation}

\begin{equation}
    \begin{split}
        \mathbb{E}\left\{ \left| \sum\limits_{m \in {\mathcal{M}}_k} w_{m,k}\sqrt{a_{m,k'}}\mathbf{\widetilde q}^H_{m,k}\boldsymbol{\Delta}_{m,k'}^{\frac{1}{2}} \mathbf{\widetilde h}_{m,k'} \right|^2\right\} &= \sum\limits_{m \in \mathcal{M}_k} w^2_{m,k}a_{m,k'}\mathbb{E}\{\mathbf{\widetilde q}^H_{m,k} \boldsymbol{\Delta}_{m,k'}^{\frac{1}{2}}\mathbf{\widetilde h}_{m,k'}\mathbf{\widetilde h}^H_{m,k'}\boldsymbol{\Delta}_{m,k'}^{\frac{1}{2}}\mathbf{\widetilde q}_{m,k} \} \\
        & = \sum\limits_{m \in \mathcal{M}_k} w^2_{m,k}\tau p^p_k a_{m,k'}\text{tr}\{\boldsymbol{\Delta}_{m,k'}\mathbf{R}_{m,k}\boldsymbol{\Psi}_{m,k} \mathbf{R}_{m,k}\}.
    \end{split}
\end{equation}


 If  the \(k'\)-th user share the same pilot with the user \(k\), i.e., \(\{k,k'\} \in \mathcal{P}_k\), then \(\mathbf{\hat h}_{m,k}\) and \(\mathbf{h}_{m,k'}\) are correlated, and we have
\begin{equation}
\label{MRC_UIkk2}
\begin{split}
 &\mathbb{E} \left( {{{\left| {{\rm{U}}{{\rm{I}}_{k,k'}}} \right|}^2}} \right)\\
 =  &\mathbb{E} \left\{ {{{\left| {\sum\limits_{m \in {\mathcal{M}}_k} w_{m,k}{\sqrt {p_{k'}^d} {{\left( {{{{\bf{\hat h}}}_{m,k}}} \right)}^H}{{\bf{h}}_{m,k'}}} } \right|}^2}} \right\} \\
   =& {p_{k'}^d}\Big( \sum\limits_{m \in \mathcal{M}_k} w_{m,k}\sqrt{\bar K_{m,k}a_{m,k}\bar K_{m,k'}a_{m,k'}}\mathbf{\bar h}^H_{m,k}\mathbf{\bar{h} }_{m,k'} + w_{m,k}\sqrt{{\bar K}_{m,k'}a_{m,k'}}\mathbf{\widetilde q}^H_{m,k} \mathbf{\bar h}_{m,k'}\\
  + &w_{m,k}\sqrt{{\bar K}_{m,k}a_{m,k} a_{m,k'}} \mathbf{\bar h}^H_{m,k} \boldsymbol{\Delta}^{\frac{1}{2}}_{m,k'} \mathbf{\widetilde h}_{m,k'} +w_{m,k}\sqrt{a_{m,k'}}\mathbf{\widetilde q}^H_{m,k} \boldsymbol{\Delta}^{\frac{1}{2}}_{m,k'} \mathbf{\widetilde h}_{m,k'}\Big)^2\\
   =&  p^d_{k'} \left|\sum\limits_{m \in {\mathcal{M}}_k}w_{m,k} \sqrt{\bar K_{m,k}\bar K_{m,k'}a_{m,k}a_{m,k'}}\mathbf{\bar h}^H_{m,k}\mathbf{\bar h}^H_{m,k'}\right|^2 + p^d_{k'} \mathbb{E}\left\{ \left| \sum\limits_{m \in \mathcal{M}_k} w_{m,k}\sqrt{\bar K_{m,k'}a_{m,k'}}\mathbf{\widetilde q}^H_{m,k}\mathbf{\bar h}_{m,k'}\right|^2\right\} \\
  + &  p^d_{k'} \mathbb{E}\left\{ \left|\sum\limits_{m \in {\mathcal{M}}_k}  w_{m,k}\sqrt{{\bar K}_{m,k}a_{m,k} a_{m,k'}} \mathbf{\bar h}^H_{m,k}  \boldsymbol{\Delta}^{\frac{1}{2}}_{m,k'}\mathbf{\widetilde h}_{m,k'} \right|^2\right\} +p^d_{k'} \mathbb{E}\left\{ \left| \sum\limits_{m \in {\mathcal{M}}_k} w_{m,k}\sqrt{a_{m,k'}}\mathbf{\widetilde q}^H_{m,k}  \boldsymbol{\Delta}^{\frac{1}{2}}_{m,k'}\mathbf{\widetilde h}_{m,k'} \right|^2\right\}\\
  +& 2 p^d_{k'} \text{Re}\left\{ \sum\limits_{m \in \mathcal{M}_k}\sum\limits_{n \in \mathcal{M}_k} w_{m,k}w_{n,k}\sqrt{\bar K_{m,k}a_{m,k}\bar K_{m,k'}a_{m,k'} a_{n,k'}}\mathbb{E}\{\mathbf{\bar h}^H_{m,k}\mathbf{\bar{h} }_{m,k'} \mathbf{\widetilde h}^H_{n,k'} \boldsymbol{\Delta}^{\frac{1}{2}}_{n,k'}\mathbf{\widetilde q}_{n,k}\} \right\}.
 \end{split}
 \end{equation}
In the following, we calculate the terms in (\ref{MRC_UIkk2}). The second and third terms are derived, and thus we derive the term \( \mathbb{E}\left\{ \left| \sum\limits_{m \in {\mathcal{M}}_k} w_{m,k}\sqrt{a_{m,k'}}\mathbf{\widetilde q}^H_{m,k}  \boldsymbol{\Delta}^{\frac{1}{2}}_{m,k'}\mathbf{\widetilde h}_{m,k'} \right|^2\right\}\), which is given by
\begin{equation}
\label{UIKK2c}
    \begin{split}
    &\mathbb{E}\left\{ \left| \sum\limits_{m \in {\mathcal{M}}_k} w_{m,k}\sqrt{a_{m,k'}}\mathbf{\widetilde q}^H_{m,k}  \boldsymbol{\Delta}^{\frac{1}{2}}_{m,k'}\mathbf{\widetilde h}_{m,k'} \right|^2\right\}\\
    =& \sum\limits_{m \in {\mathcal{M}}_k}\sum\limits_{n \in {\mathcal{M}}_k} w_{m,k}w_{n,k}\sqrt{a_{m,k'}a_{n,k'}}\mathbb{E}\{\mathbf{\widetilde q}^H_{m,k}  \boldsymbol{\Delta}^{\frac{1}{2}}_{m,k'}\mathbf{\widetilde h}_{m,k'}\mathbf{\widetilde h}^H_{n,k'}  \boldsymbol{\Delta}^{\frac{1}{2}}_{n,k'}\mathbf{\widetilde q}_{n,k}\} \\
    =& \sum\limits_{m \in {\mathcal{M}}_k}\sum\limits_{n \neq m} w_{m,k}w_{n,k}\sqrt{a_{m,k'}a_{n,k'}}\mathbb{E}\{\mathbf{\widetilde q}^H_{m,k}  \boldsymbol{\Delta}^{\frac{1}{2}}_{m,k'}\mathbf{\widetilde h}_{m,k'}\mathbf{\widetilde h}^H_{n,k'} \boldsymbol{\Delta}^{\frac{1}{2}}_{n,k'} \mathbf{\widetilde q}_{n,k} \}\\
    &+  \sum\limits_{m \in {\mathcal{M}}_k} w^2_{m,k}a_{m,k'} \mathbb{E}\{\mathbf{\widetilde q}^H_{m,k} \boldsymbol{\Delta}^{\frac{1}{2}}_{m,k'} \mathbf{\widetilde h}_{m,k'}\mathbf{\widetilde h}^H_{m,k'}  \boldsymbol{\Delta}^{\frac{1}{2}}_{m,k'}\mathbf{\widetilde q}_{m,k}\}\\ 
    \end{split}
\end{equation}

The first term in (\ref{UIKK2c}) is given by 
\begin{equation}
    \begin{split}
       & \mathbb{E}\{\mathbf{\widetilde q}^H_{m,k}  \boldsymbol{\Delta}^{\frac{1}{2}}_{m,k'}\mathbf{\widetilde h}_{m,k'}\mathbf{\widetilde h}^H_{n,k'} \boldsymbol{\Delta}^{\frac{1}{2}}_{n,k'} \mathbf{\widetilde q}_{n,k} \} \\
        =& \tau^2 p^p_k p^p_{k'}\sqrt{a_{m,k'}a_{n,k'}} \text{tr}\{ \boldsymbol{\Delta}_{m,k'} \mathbf{R}_{m,k}\boldsymbol{\Psi}_{m,k} \}  \text{tr}\{ \boldsymbol{\Delta}_{n,k'} \mathbf{R}_{n,k}\boldsymbol{\Psi}_{n,k} \} .
    \end{split}
\end{equation}

The second term in (\ref{UIKK2c}) can be calculated as
\begin{equation}
    \begin{split}
    & \mathbb{E}\{\mathbf{\widetilde q}^H_{m,k} \boldsymbol{\Delta}^{\frac{1}{2}}_{m,k'} \mathbf{\widetilde h}_{m,k'}\mathbf{\widetilde h}^H_{m,k'}  \boldsymbol{\Delta}^{\frac{1}{2}}_{m,k'}\mathbf{\widetilde q}_{m,k}\}\\
         = &\left| \Big( \sqrt{\tau p_k^p}\mathbf{R}_{m,k}\boldsymbol{\Psi}_{m,k}\sum_{j \in \mathcal{P}_k}\sqrt{\tau p^p_j a_{m,j}}\boldsymbol{\Delta}^{\frac{1}{2}}_{m,j}\mathbf{\widetilde h}_{m,j} +{\bf{n}}_{m,k}^p \Big)^H \boldsymbol{\Delta}^{\frac{1}{2}}_{m,k'}\mathbf{\widetilde h}_{m,k'}\right|^2 \\
    %= & \tau p_k^p \left| \Big(\sum_{j \in \mathcal{P}_k}\sqrt{\tau p^p_j a_{m,j}}\mathbf{\widetilde h}_{m,j} +{\bf{n}}_{m,k}^p \Big)^H \mathbf{\widetilde h}^H_{m,k'}\right|^2 \\
    =&  \tau p_k^p \mathbb{E}\left\{\sum_{j \in \mathcal{P}_k} \tau p^p_ja_{m,j} \mathbf{\widetilde h}^H_{m,j}\boldsymbol{\Delta}^{\frac{1}{2}}_{m,j} \boldsymbol{\Psi}_{m,k}\mathbf{R}_{m,k} \boldsymbol{\Delta}^{\frac{1}{2}}_{m,k'}\mathbf{\widetilde h}_{m,k'}\mathbf{\widetilde h}^H_{m,k'}\boldsymbol{\Delta}^{\frac{1}{2}}_{m,k'}\mathbf{R}_{m,k}\boldsymbol{\Psi}_{m,k}\boldsymbol{\Delta}^{\frac{1}{2}}_{m,j}\mathbf{\widetilde h}_{m,j} \right\} \\
    &+ \tau p_k^p |{(\bf{n}}_{m,k}^p)^H\boldsymbol{\Psi}_{m,k}\mathbf{R}_{m,k} \boldsymbol{\Delta}^{\frac{1}{2}}_{m,k'} \mathbf{ \widetilde h}_{m,k'}|^2 \\
    = & \tau p_k^p \sigma^2 \text{tr}\{\boldsymbol{\Psi}_{m,k}\mathbf{R}_{m,k} \boldsymbol{\Delta}_{m,k'}\mathbf{R}_{m,k}\boldsymbol{\Psi}_{m,k}\} \\
    +& \tau p_k^p \sum\limits_{j \in \mathcal{P}_k}\tau p^p_j a_{m,j}\text{tr}\{ \boldsymbol{\Delta}_{m,j}\boldsymbol{\Psi}_{m,k}\mathbf{R}_{m,k} \boldsymbol{\Delta}_{m,k'}\mathbf{R}_{m,k}\boldsymbol{\Psi}_{m,k}\} \\
    +& \tau^2 p_k^p p_{k'}^pa_{m,k'}\text{tr}\{\boldsymbol{\Delta}_{m,k'}\boldsymbol{\Psi}_{m,k}\mathbf{R}_{m,k} \}\text{tr}\{\boldsymbol{\Delta}_{m,k'}\boldsymbol{\Psi}_{m,k}\mathbf{R}_{m,k} \} \\
    = &\tau^2 p_k^p p_{k'}^pa_{m,k'} \text{tr}\{\boldsymbol{\Delta}_{m,k'}\boldsymbol{\Psi}_{m,k}\mathbf{R}_{m,k} \}\text{tr}\{\boldsymbol{\Delta}_{m,k'}\boldsymbol{\Psi}_{m,k}\mathbf{R}_{m,k} \} + \tau p_k^p \text{tr}\{\mathbf{R}_{m,k} \boldsymbol{\Delta}_{m,k'}\mathbf{R}_{m,k}\boldsymbol{\Psi}_{m,k}\} .   
    \end{split}
\end{equation}

\(\mathbb{E}\{\mathbf{\bar h}^H_{m,k}\mathbf{\bar{h} }_{m,k'} \mathbf{\widetilde h}^H_{n,k'} \boldsymbol{\Delta}^{\frac{1}{2}}_{n,k'}\mathbf{\widetilde q}_{n,k}\}\) can be calculated as
\begin{equation}
    \begin{split}
        \mathbb{E}\{\mathbf{\bar h}^H_{m,k}\mathbf{\bar{h} }_{m,k'} \mathbf{\widetilde h}^H_{n,k'} \boldsymbol{\Delta}^{\frac{1}{2}}_{n,k'}\mathbf{\widetilde q}_{n,k}\} =  \tau\sqrt{ p^p_{k'}p^p_{k}a_{n,k'}} \mathbf{\bar h}^H_{m,k}\mathbf{\bar{h} }_{m,k'} \text{tr}\{\boldsymbol{\Delta}_{n,k'}\mathbf{R}_{n,k}\boldsymbol{\Psi}_{n,k}\}.
    \end{split}
\end{equation}



The term $\mathbb{E}\left( \left| {{\rm{LS}}_{k}} \right|^2 \right)$ is given by
\begin{equation}
\setlength\abovedisplayskip{5pt}
\setlength\belowdisplayskip{5pt}
\label{MRC_LSk}
\begin{split}
&\mathbb{E} \left\{ {{{\left| {{\rm{LS}}_{k}} \right|}^2}} \right\}  
= {p_k^d} \mathbb{E} \left\{ {{{\left| {\sum\limits_{m \in {\mathcal{M}}_k}{{{\left( {{\bf{\hat h}}_{m,k}} \right)}^H}{\bf{h}}_{m,k} } -  {{\rm{DS}}_{k}}} \right|}^2}} \right\}   \\
%=& p^d_k \mathbb{E}\{ |\sum\limits_{m \in \mathcal{M}_k}\mathbf{\widetilde h}^H_{m,k}\mathbf{\widetilde h}_{m,k}|^2\} + p^d_k \mathbb{E}\{ |\sum\limits_{m \in \mathcal{M}_k}\mathbf{\widetilde h}^H_{m,k}\mathbf{\widetilde e}_{m,k}|^2\} -{{\rm{DS}}^2_{k}}\\
= &{p_k^d}\Big(\sum\limits_{m \in {\mathcal{M}}_k} w_{m,k}\sqrt{\bar K_{m,k}a_{m,k}}\mathbf{\widetilde q}^H_{m,k} \mathbf{\bar{h} }_{m,k} + w_{m,k}\sqrt{\bar K_{m,k}a_{m,k}a_{m,k}} \mathbf{\bar{h} }^H_{m,k}\boldsymbol{\Delta}_{m,k}^{\frac{1}{2}}\mathbf{\widetilde{h} }_{m,k}\\
 & +w_{m,k}\sqrt{a_{m,k}}\mathbf{\widetilde q}^H_{m,k}\boldsymbol{\Delta}_{m,k}^{\frac{1}{2}}\mathbf{\widetilde{h} }_{m,k} - {w_{m,k}}\tau p^p_k \text{tr}\{\mathbf{R}_{m,k}\boldsymbol{\Psi}_{m,k}\mathbf{R}_{m,k}\}\Big)^2 \\
 =& {p_k^d} \sum\limits_{m \in {\mathcal{M}}_k} w^2_{m,k}\bar K_{m,k}a_{m,k} \mathbb{E}\{|\mathbf{\widetilde q}^H_{m,k}\mathbf{\bar{h} }_{m,k} |^2\} + {p_k^d} \sum\limits_{m \in {\mathcal{M}}_k}  w^2_{m,k}\bar K_{m,k}a_{m,k}a_{m,k} \mathbb{E}\{|\mathbf{\bar{h} }^H_{m,k}\boldsymbol{\Delta}_{m,k}^{\frac{1}{2}}\mathbf{\widetilde{h} }_{m,k} |^2\}\\
  &+  {p_k^d} \mathbb{E}\left\{ \sum\limits_{m \in {\mathcal{M}}_k}\sum\limits_{n \in {\mathcal{M}}_k} w_{m,k}w_{n,k}\sqrt{a_{m,k} a_{n,k}}\mathbf{\widetilde q}^H_{m,k}\boldsymbol{\Delta}_{m,k}^{\frac{1}{2}}\mathbf{\widetilde{h} }_{m,k}\mathbf{\widetilde{h} }^H_{n,k}\boldsymbol{\Delta}_{n,k}^{\frac{1}{2}}\mathbf{\widetilde q}_{n,k}\right\}\\
  &+ {p_k^d}\Big(\sum\limits_{m \in {\mathcal{M}}_k}{w_{m,k}}\tau p^p_k \text{tr}\{\mathbf{R}_{m,k}\boldsymbol{\Psi}_{m,k}\mathbf{R}_{m,k}\}\Big)^2 \\
  & - 2{p_k^d}\text{Re}\left\{\sum\limits_{m \in {\mathcal{M}}_k}\sum\limits_{n \in {\mathcal{M}}_k}  \tau p^p_k \text{tr}\{\mathbf{R}_{n,k}\boldsymbol{\Psi}_{n,k}\mathbf{R}_{n,k}\}w_{m,k}w_{n,k}\sqrt{a_{m,k}}\mathbb{E}\{\mathbf{\widetilde q}^H_{m,k}\boldsymbol{\Delta}_{m,k}^{\frac{1}{2}}\mathbf{\widetilde{h} }_{m,k}\}\right\} .
 \end{split}
\end{equation}

Then, the first term \(\mathbb{E}\{|\mathbf{\widetilde q}^H_{m,k}\mathbf{\bar{h} }_{m,k} |^2\}\) of (\ref{MRC_LSk}) can be calculated as
\begin{equation}
    \begin{split}
        \mathbb{E}\{|\mathbf{\widetilde q}^H_{m,k}\mathbf{\bar{h} }_{m,k} |^2\} = \tau p^p_k \mathbf{\bar h}^H_{m,k} \mathbf{R}_{m,k}\boldsymbol{\Psi}_{m,k}\mathbf{R}_{m,k}\mathbf{\bar h}_{m,k}.
    \end{split}
\end{equation}
The second term \(\mathbb{E}\{|\mathbf{\bar{h} }^H_{m,k}\mathbf{\widetilde{h} }_{m,k} |^2\}\) is given by
\begin{equation}
    \mathbb{E}\{|\mathbf{\bar{h} }^H_{m,k}\mathbf{\widetilde{h} }_{m,k} |^2\} = \mathbf{\bar h}^H_{m,k}\boldsymbol{\Delta}_{m,k}\mathbf{\bar h}_{m,k}.
\end{equation}
The third term in (\ref{MRC_LSk}) can be written as
\begin{equation}
\begin{split}
    &\mathbb{E}\left\{ \sum\limits_{m \in {\mathcal{M}}_k}\sum\limits_{n \in {\mathcal{M}}_k} w_{m,k}w_{n,k}\sqrt{a_{m,k} a_{n,k}}\mathbf{\widetilde q}^H_{m,k}\boldsymbol{\Delta}_{m,k}^{\frac{1}{2}}\mathbf{\widetilde{h} }_{m,k}\mathbf{\widetilde{h} }^H_{n,k}\boldsymbol{\Delta}_{n,k}^{\frac{1}{2}}\mathbf{\widetilde q}_{n,k}\right\}  \\
    =& \mathbb{E}\left\{ \sum\limits_{m \in {\mathcal{M}}_k}\sum\limits_{n \neq m}w_{m,k}w_{n,k}\sqrt{a_{m,k} a_{n,k}}\mathbf{\widetilde q}^H_{m,k}\boldsymbol{\Delta}_{m,k}^{\frac{1}{2}}\mathbf{\widetilde{h} }_{m,k}\mathbf{\widetilde{h} }^H_{n,k}\boldsymbol{\Delta}_{n,k}^{\frac{1}{2}}\mathbf{\widetilde q}_{n,k}\right\} \\
    +& \mathbb{E}\left\{ \sum\limits_{m \in {\mathcal{M}}_k} w^2_{m,k}a_{m,k}\mathbf{\widetilde q}^H_{m,k}\boldsymbol{\Delta}_{m,k}^{\frac{1}{2}}\mathbf{\widetilde{h} }_{m,k}\mathbf{\widetilde{h} }^H_{m,k}\boldsymbol{\Delta}_{m,k}^{\frac{1}{2}}\mathbf{\widetilde q}_{m,k}\right\} \\
    %=& \sum\limits_{m \in {\mathcal{M}}_k}\sum\limits_{n \neq m}(N\tau p^p_k a_{m,k}a_{n,k})^2b_{m,k}b_{n,k}  \\
    %+&  \sum\limits_{m \in {\mathcal{M}}_k}a_{m,k}\tau p^p_k a^2_{m,k}b^2_{m,k}\Big(\sum\limits_{j \in \mathcal{P}_k}\sqrt{\tau p^p_{m,j}a_{m,j}}\mathbf{\widetilde h}^H_{m,j}\mathbf{\widetilde h}_{m,k}+(\mathbf{n}^p_{m,k})^H\mathbf{\widetilde h}_{m,k}\Big)\\
    %\times & \Big(\sum\limits_{j \in \mathcal{P}_k}\sqrt{\tau p^p_{m,j}a_{m,j}}\mathbf{\widetilde h}^H_{m,j}\mathbf{\widetilde h}_{m,k}+(\mathbf{n}^p_{m,k})^H\mathbf{\widetilde h}_{m,k}\Big)^H\\
    =&  \Big(\tau p^p_k \sum \limits_{m \in \mathcal{M}_k}w_{m,k} a_{m,k}\text{tr}\{\boldsymbol{\Delta}_{m,k}\mathbf{R}_{m,k}\boldsymbol{\Psi}_{m,k}   \} \Big)^2 + \sum\limits_{m \in \mathcal{M}_k} w^2_{m,k}\tau p_k^p a_{m,k}\text{tr}\{\mathbf{R}_{m,k} \boldsymbol{\Delta}_{m,k}\mathbf{R}_{m,k}\boldsymbol{\Psi}_{m,k}\}. 
\end{split} 
\end{equation}
The fourth term \(\mathbb{E}\{\mathbf{\widetilde q}^H_{m,k}\boldsymbol{\Delta}_{m,k}^{\frac{1}{2}}\mathbf{\widetilde{h} }_{m,k}\}\) is calculated as
\begin{equation}
   \mathbb{E}\{\mathbf{\widetilde q}^H_{m,k}\boldsymbol{\Delta}_{m,k}^{\frac{1}{2}}\mathbf{\widetilde{h} }_{m,k}\} = \tau p^p_k \sqrt{a_{m,k}} \text{tr}\{\boldsymbol{\Delta}_{m,k}\mathbf{R}_{m,k}\boldsymbol{\Psi}_{m,k}\}.
\end{equation}
By substituting all terms into (\ref{MRC_LSk}), we have
\begin{equation}
    \begin{split}
        \mathbb{E} \left\{ {{{\left| {{\rm{LS}}_{k}} \right|}^2}} \right\}  & =   {p_k^d} \sum\limits_{m \in \mathcal{M}_k}w^2_{m,k} \bar K_{m,k}\tau p^p_k a_{m,k} \mathbf{\bar h}^H_{m,k} \mathbf{R}_{m,k}\boldsymbol{\Psi}_{m,k} \mathbf{R}_{m,k}\mathbf{h}_{m,k}\\
        & + p_k^d \sum\limits_{m \in \mathcal{M}_k} w^2_{m,k}\bar K_{m,k}a_{m,k}a_{m,k}\mathbf{\bar h}^H_{m,k}\boldsymbol{\Delta}_{m,k} \mathbf{\bar h}_{m,k}\\
        &+ p_k^d \sum\limits_{m \in \mathcal{M}_k} w^2_{m,k}\tau p_k^p a_{m,k}\text{tr}\{\mathbf{R}_{m,k} \boldsymbol{\Delta}_{m,k}\mathbf{R}_{m,k}\boldsymbol{\Psi}_{m,k}\}
       % &+ {p_k^d} \sum\limits_{m \in {\mathcal{M}}_k} a_{m,k} N\tau p_k^pa^2_{m,k}b_{m,k}(Nb_{m,k}\tau p^p_{k}a_{m,k}+1) \\
        %& - 2{p_k^d}\text{Re}\left\{\sum\limits_{m \in {\mathcal{M}}_k}  N \tau p^p_k a^{5/2}_{m,k}b_{m,k}N \tau p^p_{k}a^{3/2}_{m,k}b_{m,k}\right\}-
    \end{split}
\end{equation}
 %( N \tau p^p_k a^2_{m,k}b_{m,k})^2

Finally, we compute $\mathbb{E}\left( \left| {{\rm{N}}_{k}} \right|^2 \right)$, which is given by
\begin{equation}
\label{MRC_Nk}
\begin{split}
    \mathbb{E} \left( {{{\left| {{{\rm{N}}_k}} \right|}^2}} \right) &= \mathbb{E}\{|\sum\limits_{m \in \mathcal{M}_k} \sqrt{w_{m,k}} {{{\left( {{\bf{ \hat h}}_{m,k}} \right)}^H}{\bf{n}}_m}|^2\} \\
        & = \sum\limits_{m \in \mathcal{M}_k}{w^2_{m,k}}\Big( \tau p^p_k  \text{tr}\{\mathbf{R}_{m,k}\boldsymbol{\Psi}_{m,k}\mathbf{R}_{m,k}\} + \bar K_{m,k}a_{m,k} \mathbf{\bar h}^H_{m,k}\mathbf{\bar h}_{m,k}\Big)\sigma^2 .
\end{split}
\end{equation}

Substituting all these results into (\ref{kth_SINR}), we obtain \(1 \) in (\ref{MRC_SINR_LB}).
\end{appendices}
